CAN Radar: Sensing Physical Devices in CAN Networks based on Time Domain Reflectometry

The presence of security vulnerabilities in automotive networks has already been shown by various publications in recent years. Due to the specification of the Controller Area Network (CAN) as a broadcast medium without security mechanisms, attackers are able to read transmitted messages without being noticed and to inject malicious messages. In order to detect potential attackers within a network or software system as early as possible, Intrusion Detection Systems (IDSs) are prevalent. Many approaches for vehicles are based on techniques which are able to detect deviations from specified CAN network behaviour regarding protocol or payload properties. However, it is challenging to detect attackers who secretly connect to CAN networks and do not actively participate in bus traffic. In this paper, we present an approach that is capable of successfully detecting unknown CAN devices and determining the distance (cable length) between the attacker device and our sensing unit based on Time Domain Reflectometry (TDR) technique. We evaluated our approach on a real vehicle network.

==> countermeasures.tex <==
\subsection{Countermeasures}
\label{sec:countermeasures}
In general, software should be designed from the ground up as secure as possible by applying \textit{security by design} during the development process. There are several \textit{security principles}, which software architects should consider. The following countermeasures are only examples for our observed target based on the mentioned principles. 

\subsubsection{Selection of Suitable Technologies}
Documented exploitation of passenger vehicles was achieved in multiple cases by sending or replaying \ac{CAN} messages on the target's bus. \ac{CAN} can be seen as a bus system not designed with security issues in mind. Techniques like \emph{threat modeling}~\cite{Microsoft.2005}\cite{Durrwang.2017} could provide valuable information before the actual implementation and address these issues in advance. Moreover, choosing the optional deployment methods using an \ac{ACL} during the design phase could have prevented the exploitation via \ac{CAN} only.

\subsubsection{Hard-wired Plausibility Checks}
The connector of our target was designed to accommodate over 100 \emph{pins}. Although the presence of pins depends on the exact model the target is installed in, this high number is explained by the presence of physical signals being directly connected to the target. Besides the obvious need for \emph{hard-wired connections}, e.g., the connection to the pyrotechnic charges, it was discovered that signals such as \emph{seatbelt status} and \emph{seat occupancy} were connected as well. While this does not exclude the possibility of information being transmitted over a bus system as well, this would allow for plausibility checks based on sources that are not easy to be tampered with~\cite{vehicular2017}.

\subsubsection{Usage of Cryptography}
\label{subsec:use_crypt}
When developers want to design a new security feature, they should follow the \textit{Kerckhoff's Principle}. The principle explicitly describes that cryptosystems shouldn't be secure due to hidden details about how the algorithm works (security by obscurity). Moreover, the whole secret should be based on the confidentiality of the utilized key. The past has already shown multiple times that mechanisms which disregard the mentioned principle are very often broken as soon as the algorithm has been reverse-engineered~\cite{Pelzl_Paar}. Our investigation has also confirmed the violation of the mentioned principle by analyzing the sent seed. A first approach to fix the existing issue could be an additional security layer which ensures a correct authentication.

\subsubsection{Hardening Against Brute-Force Attacks}
\label{subsec:HardeningAgainstBruteForceAttacks}
The use of \acp{NRC}, such as \emph{exceeded number of attempts} and \emph{required time delay not expired}, as described in the UDS standard could be used to slow down brute-force attempts. While the former would require a power cycle of the \emph{target} to continue the brute-force attempt, the latter would slow the approach down. To counter the use of scripted power cycling of the target in rapid succession, the target could require a certain time delay after being powered on before enabling the diagnostic \ac{EOL} capability.

The length of the \emph{seed} and \emph{key} could be increased to harden the target against brute-force attempts. As mentioned before the length of 2 bytes leads to 65536 possible \emph{keys} per \emph{seed}. By using the MSB for the version number of the implemented \ac{ISO} standard, the MSB is fixed in every \emph{seed}. Thus, by only changing the values of the LSB, only 256 different \emph{seeds} can be supplied by the target after a request, albeit being 16 bit long. Although, the amount of possible \emph{keys} per \emph{seed} is 65536, because it is 16 bit long, this reduces the amount of maximum tries to unlock the \emph{Security Access}, as the same \emph{seeds} occur more frequently, making it faster to iterate the possible \emph{keys}.


\subsubsection{Stateful Firewalls}
The execution of diagnostic functionality in general should only be allowed in their corresponding vehicle states. However, our evaluation has shown, that this simple guideline is not always implemented correctly. For instance, in one of our tested vehicles, the gateway did not check for the appropriate conditions, before performing certain diagnostic functions. As a consequence of this, diagnostic functions are available during vehicle conditions in which there would be malicious applications for them. This includes entering a diagnostic session specifically for safety systems, e.g., airbags, at highway speeds. Furthermore, it is probable that even more implementation flaws exist in our target that have yet to be discovered. Thus, it would be sensible to filter diagnostic requests reliably depending on the actual vehicle state before they can reach the destined \ac{ECU} itself. A concrete and more effective approach is the implementation of a stateful firewall in the gateway, inspecting the messages depending on the current vehicle state. At this point, it would be conceivable to use existing hard-wired sensors to provide data for additional plausibility checks to ensure that the vehicle state can be determined correctly.


==> existent_attacks.tex <==
\section{Automotive vulnerability database and existent attacks}
\label{sec:existent_attacks}
This section shows a classification of existent attacks and one possible approach for automotive vulnerability database. We decided to put these two points into public, in hope to help other researches, to initiate a process of a common exchange of automotive vulnerabilities and to present found attacks.

\subsection{Attack classification}
\label{subsec:attack_class}

%Abbildung beschreiben: Notation, auf die Häufigkeit eingehen
As mentioned in the earlier section, a significant number of automotive attacks exist in publications with a growing number of researches. But unfortunately there is no summary or classification presented. Therefore we have collected the available published information to construct a vulnerability catalogue which includes successfully performed attacks. Six classes were used into which the found attacks were sorted. For this purpose an existent taxonomy is used where the notation is a derivative approach of the \ac{CERT}~\cite{CERT.,ENISA.2015}.

\textit{Malicious code} refers to input or uploading of modified or malicious code on the target. This can be done by writing a modified firmware or malicious code to an ECU using its update functionality.

\textit{Intrusion attempts} describes exploiting vulnerabilities like the absent of a length check in a function that deals with data (buffer overflow). Here, targeted memory cells were overridden to alter the behaviour of a system.

\textit{Fraud} means gaining advantages by stealing information from a system. This can be done by the extraction of firmware, stealing secrets or extracting private data from a car. Additionally this class is related to key-less entry attacks where information is transmitted over a greater distance to fake the key’s position. This is useful to fake location information like position of the key and thus open a car even when its owner is hundreds of meters away.

\textit{Intrusion} describes in our case, the triggering or application of existing functions in a way that the target system acts unordinary. In the automotive context this is e.g. misuse of standard functions. Therefore manipulated data can be used to bring a system in a harmful condition state. Exemplary is triggering of a diagnostic function like brake bleed while the vehicle is in motion.

\textit{Information security} describes the act of gaining of unauthorized access to a system. For example, this can be done by bypassing a protection like an encryption.

Un-\textit{Availability} describes any method which leads to the unavailability of a service, function or host. In most cases a \ac{DoS} attack is used where the network is flooded with a huge number of requests.

The bar chart (Figure~\ref{fig:attacks}) presents our summary of automotive attacks. The filled grey bars show attacks found in publications while the patterned ones represent attacks that are found in this research work.
\begin{figure}[!ht]
\begin{center}
\include{bar_chart_attacks}
\end{center}
\vspace{-5ex}
	\caption{Occurrence of automotive attacks in science \cite{Checkoway.2011,Koscher.2010,IshtiaqRoufaRobMillerb.2010,Miller.2013,Hoppe.2011,Poulsen.2010,Francillon.2011,Bacchus.2014,Kim.2013,Spaar.2015,Craig.2014,Schroder.2013,Howard.2012,Bailey.2011,Charlie.2015} (attacks which are done by us are marked with gray patterns).}
	\label{fig:attacks}
\end{figure}

As illustrated in Figure~\ref{fig:attacks}, the classes \textit{malicious code, fraud} and \textit{intrusion} have the highest occurrence. Moreover the class \textit{intrusion} with a number of 35 published attacks, represents by far the most important attack class. It also includes the most dangerous threats against a car's safety. Accordingly the search was focused on such attacks in the analysis and 5 attacks were found while attacking vehicles from two premium car manufacturers. The high number of attacks in this class can be explained with the open standards like \ac{UDS}, \ac{OBD} and \ac{KWP}. They provide sufficient information to easily start an attack against a car. But to become a safety critical attack, plausibility or authentications have to be absent. Unfortunately in most cars these mechanisms are absent or they are badly implemented e.\,g., \cite{Ring.2014}. If these mechanisms are missing, an attacker can execute diagnostic functions while a car is moving instead of standing still like it is supposed to be by the \acp{OEM}. This misuse of diagnostic functions can lead to dangerous situations like losing braking power.
\pagebreak
